Confluent-Drawing Parallel Coordinates: Web-Based Interactive Visual Analytics of Large Multi-Dimensional Data

Parallel coordinates plot is one of the most popular and widely used visualization techniques for multi-dimensional data sets. Its main challenges for large-scale data sets are visual clutter and overplotting which hamper the recognition of patterns and trends in the data. In this paper, we propose a confluent drawing approach of parallel coordinates to support the web-based interactive visual analytics of large multi-dimensional data. The proposed method maps multi-dimensional data to node-link diagrams through the data binning-based clustering for each dimension. It uses density-based confluent drawing to visualize clusters and edges to reduce visual clutter and overplotting. Its rendering time is independent of the number of data items. It supports interactive visualization of large data sets without hardware acceleration in a normal web browser. Moreover, we design interactions to control the data binning process with this approach to support interactive visual analytics of large multi-dimensional data sets. Based on the proposed approach, we implement a web-based visual analytics application. The efficiency of the proposed method is examined through experiments on several data sets. The effectiveness of the proposed method is evaluated through a user study, in which two typical tasks of parallel coordinates plot are performed by participants to compare the proposed method with another parallel coordinates bundling technique. Results show that the proposed method significantly enhances the web-based interactive visual analytics of large multi-dimensional data.

==> body.tex <==
%-------------------------------------------------------------------------
\section{Introduction}

%Visual analytics is a method to synthesize information and derive insight from massive, dynamic, ambiguous, and often conflicting data; detect the expected and discover the unexpected; provide timely, defensible, and understandable assessments; and communicate assessment effectively for action by combining human judgment \cite{Thomas2006}. 

Visual analytics is the science of analytical reasoning facilitated by interactive visualization \cite{Thomas2006}. It integrates human perception, cognition, and reasoning abilities into the data analysis process through visualization and interactions. With the explosion of data, one of its main challenges is to develop scalable interactive visualization techniques for large-scale data to reduce the growing impedance mismatch between data volume/complexity and the human ability to explore and interact with data.

To address this challenge with a focus on data presentation, many techniques have been proposed for exploratory visualization of multi-dimensional data, targeted at both generic and specific application domains \cite{Ware2004,Keim2002}. Parallel coordinates plot (PCP) has become a standard tool for visualizing multi-dimensional data \cite{Heinrich2013}. It has been incorporated into several visual analytics applications, including iPCA \cite{Jeong2009} and iVisClassifier \cite{Choo2010}. In PCPs, axes, that corresponding to dimensions of the original data, are aligned parallel to each other and data points are mapped to lines intersecting the axes at the respective value. The embedding of an arbitrary number of parallel axes into the plane allows the simultaneous display of many dimensions, providing a good overview of the data. However, with classic PCP, although the representation of data points as lines may reveal trends and patterns contained in the data, it also tends to create visual clutter caused by overplotting, especially for large-scale data sets. This visual clutter is one of the main challenges of PCP, which hamper the recognition of patterns in the data. Furthermore, the zigzagging polygonal lines (polylines) used for data representation leads to the cross-over problem, which generally loose visual continuation across the axes in PCP, because they are only $C^{0}$ continuous \cite{Luo2008}. With the cross-over problem, users are difficult to follow lines that share a common point along an axis. 

Edge-bundling is a widely used approach to reduce visual clutter in PCP. The data will be aggregated first with data clustering algorithms, then rendered in an illustrative fashion using different forms of edge-bundling or to distinguish between major trends and outliers. However, existing data clustering and edge-bundling techniques used in PCP are not scalable well for large-scale data. Their computing performance depends on the number of dimensions and data points. Their rendering performance depends on the number of lines. This significantly hinders the integration of human judgment into the data analysis process because they have been too slow for interactive use when the number of dimensions or the volume of data sets is scaled up. Furthermore, without human judgment, the clusters generated by automatic algorithms may not reveal the real trends and patterns in the data.
%, which leads to that clusters and related internal structure of the data are not represented in the geometry of the plot.

In this paper, we propose an edge-merging PCP technique for large-scale data sets, which includes a one-dimensional clustering method and an edge-merging layout for PCPs. It is scalable for large-scale data sets and supports interactive use in the visual analytics process with acceptable near-real-time performance. The experiments on several data sets are conducted to demonstrate the effectiveness of our edge-merging PCP technique. Our edge-merging PCP technique enhances the visual analytics for large-scale multi-dimensional data sets in the following ways:
%web-based visual analytics framework for large-scale data sets, which uses an edge-merging layout for parallel coordinates plot. The framework enhances the visual analytics for large-scale data sets in the following ways:
\begin{enumerate}
	\item It uses a one-dimensional clustering method to cluster the data in each dimension independently. The clusters are shown on each axis. The clustering is highly configurable, including configuring the number and the size of the clusters, to integrate human judgment in the visual analytics process.
	\item It reduces the number of lines that need to be rendered by merging the lines belong to the same clusters in two neighboring axes together as one single B\'ezier spline. This edge-merging layout reduces the rendering time. It makes the rendering process scalable for large-scale data sets since the rendering performance is independent of the number of data points. 
	\item To overcome the cross-over problem, it renders the merged lines as B\'ezier splines.
	\item It computes the densities of merged lines to render their widths to reveal the trends, patterns and data distributions between axes.
	%To reveal the internal structure and the data distribution between axes, it computes the density of each merged line and uses the density to render the width of the line.
	%To improve the visual analytics process, according to users' interactions, it supports to only visualize the selected dimensions of a data set instead of all dimensions.
\end{enumerate}
Based on the edge-merging PCP, we implement a web-based visual analytics application. The application enhances the visual analytics for large-scale multi-dimensional data sets in the following ways:
\begin{enumerate}
	\item Its web-based architecture separates the rendering process and clustering process. The clustering process is performed on the server side. The clustering result is rendered in browsers, which supports the interactive exploration of large-scale data with an edge-merging PCP.
	%and can be integrated with big data platforms, for example, Apache Hadoop, through web services to improve the computing performance.
	\item The application integrates human perception and reasoning abilities into the data analysis process by supporting the configuration of the clustering in each axis to continuously improve the visualization results.
\end{enumerate}

%It shows that the merged B\'ezier splines between clusters maintain the users' ability to recognize the correlation between dimensions. Furthermore, it uses the width of the merged curves for revealing the internal structure and the data distribution between two axes, which leaves the color perceptual channel free for visualizing other attributes. 
%The rendering performance of the framework is evaluated by comparing its rendering time with classic PCP. This comparison is conducted based on several different data sets. It shows that this framework allows fast construction of merged curves while guaranteeing a good overview of high-dimensional data sets, especially for large-scale data sets.

The paper is organized as follows: Section~\ref{section:related work} reviews related work. Section~\ref{section:method} presents the method used in the proposed visual analytics framework. Section~\ref{section:experiment} conducts the experiments and Section~\ref{section:discussion} discusses the result. Section~\ref{section:future} draws conclusions and discusses future work.

%discusses the case studies and the evaluation of the rendering performance of the framework.

\section{Related Work}\label{section:related work}

Since parallel coordinates were introduced in the seminal work of Inselberg \cite{inselberg1985plane,inselberg1987parallel}, and later extended by Wegman \cite{wegman1990hyperdimensional} as a visualization tool, it has become a common and widely used visualization technique for visualizing high-dimensional data. It aligns parallel axes to each other and data points are mapped to coordinates intersecting the axes at the respective value. It allows the simultaneous display of a number of dimensions by embedding of the corresponding number of parallel axes into a plane to reveal trends and patterns in the data.

For large data sets, visual clutter caused by heavy overplotting of lines is often cited as a major challenge for parallel coordinates \cite{Heinrich2013}. Preprocessing the data with various clustering algorithms is a possible approach to reduce the visual clutter \cite{jain1988algorithms}. The clusters can then be displayed and highlighted in extensions of PCPs by using color or edge-bundling. Fua et al. \cite{fua1999hierarchical} develop a multiresolutional view of the data via hierarchical clustering, and use a variation on parallel coordinates to convey aggregation information for the resulting clusters. To reveal details of the internal structure of clusters, Johansson et al. \cite{johansson2005revealing} combine clusters and high-precision textures in a PCP to represent data, in which specific transfer functions that operate on the high-precision textures are used to highlight different aspects of the cluster characteristics. These clusters generated by multidimensional clustering algorithms may not reflect the relation between the two axes because not all dimensions have a strong correlation. Palmas et al. \cite{Palmas2014} present an edge-bundling layout for PCPs using density-based clustering for each dimension independently so that the clustering is directly related to the shown dimensions in every part of the plot. However, these clustering methods are not suitable for a visual analytics application because they are not configurable: the number or size of clusters is generated automatically by algorithms. In contrast, our edge-merging technique takes advantage of human expertise by supporting the configuration of the number and size of clusters. Furthermore, existing clustering-based PCPs are not scalable for large-scale data. The long computation time makes them too slow for interactive use in the visual analytics process. For example, in Palmas et al.'s \cite{Palmas2014} method, to reduce the computation time for the clustering, they sample the parameters 2000 times between 25\% and 1\% of the data range instead of computing it on the whole data range. However, this precomputation still needs almost one minute for $10^{5}$ data points on current desktop hardware in a single computing thread. We propose a one-dimensional clustering method to cluster the data in each dimension independently, which reduces much computation time.

The edge-bundling method that uses cubic B-splines to show adjacency relations atop different tree visualization methods was proposed for the first time by Holten et al. \cite{holten2006hierarchical}.  It has been adapted to PCPs based on data clustering by McDonnell et al. \cite{McDonnell2008}. With edge bundling, polylines in PCP become polycurves, which are bent between two axes towards centroid of the corresponding clusters. While this approach reduces visual clutter by freeing up screen space, the resulting polycurves are still $C^{0}$ continuous, which makes them difficult to be visually traced. To avoid this, Heinrich et al. \cite{heinrich2011evaluation} use a $C^{1}$ continuous bundling. Furthermore, Zhou et al. \cite{Zhou2008} present a bundling method that creates visual clusters without the prerequisite of data clustering. However, the bundling brings the curves closer to each other, which may increase the overplotting within a bundle and hide the internal structure of clusters \cite{Palmas2014}. In addition, its rendering performance depends on the number of curves, which hinders the interactive exploration for large-scale data. To reduce the overplotting in bundles and make the rendering performance independent of the number of data points, we propose an edge-merging layout for PCP by combining the idea of confluent drawing and edge bundling. Confluent drawing \cite{dickerson2003confluent} merges groups of edges and draws them as tracks, which allows even very dense and non-planar graphs to be drawn in a planar way. It was first proposed for node-link diagrams. Figure~\ref{fig:cd} illustrates the visual improvement of a simple confluent drawing over the corresponding node-link diagram. Our edge-merging method merges bundles between clusters in the same way.

\begin{figure}[htb]
	\centering
	\begin{subfigure}{0.45\linewidth}
		\centering
		\includegraphics[width=.45\linewidth]{imgs/cd1}
		\caption{\label{fig:cd1}
			\textit{A graph drawn as a traditional node-link diagram.}} 
	\end{subfigure}
	\hspace*{\fill} 
	\begin{subfigure}{0.45\linewidth}
		\centering
		\includegraphics[width=.45\linewidth]{imgs/cd2}
		\caption{\label{fig:cd2}
			\textit{The same graph, with confluent drawing.}}
	\end{subfigure}
	
	\caption{\label{fig:cd}
		\textit{The visual improvement of a simple confluent drawing over the corresponding node-link diagram} \cite{Eppstein2016}.}
\end{figure} 

Another popular solution to the overplotting problem is to replace opaque lines with a density representation in PCPs \cite{miller1991construction, wegman1997high}. Artero et al. \cite{Artero2004} highlight significant relationships between axes in a PCP by constructing a density plot based on density information computed from the data set. Heinrich et al. \cite{Heinrich2009} derive a mathematical density model to generate a continuous parallel coordinates plot. To reveal the internal structure of clusters and the data distribution between axes, we compute the densities of merged bundles to render their widths. It is effective even with a purely geometry-based visualization, which leaves the color and opacity perceptual channels free for visualizing other information.

%To summarize, our contribution in this work is a flexible visual analytics technique that uses a combination of previously proposed techniques: PCP with clustering for each axis independently, and the edge-merging layout. In addition, we allow user-configured clusters for each data dimension. To the best of our knowledge, we are the first to propose such technique.

% This is a repetition from Introduction, no need for it
% Visual analytics is the science of analytical reasoning facilitated by interactive visual interfaces \cite{Thomas2006}. It uses visualization as a medium and interaction as a mean to integrate human perception, cognition, and reasoning abilities into the data analysis process. PCP has been incorporated into several visual analytics applications, including iPCA \cite{Jeong2009} and iVisClassifier \cite{Choo2010}, to gain insight into high-dimensional data sets. However, they are not scalable for extreme large-scale data sets and designed for specific problem domains. In contrast, we develop a general visual analytics framework for large-scale high-dimensional data sets based on the edge-merging layout for PCP. 

\section{Method} \label{section:method}

With our edge-merging PCP technique, the data for each dimension is clustered based on a one-dimensional clustering method which is evolved from K-means clustering (Section~\ref{section:dataclustering}). The data points between axes are merged together according to the clusters in each axis (Section~\ref{section:edgemerging}). The merged data points are rendered as B\'ezier splines with specific widths which are determined by their densities (Section~\ref{section:representation}). Our technique is implemented as a web-based visual analytics application with an intention to integrate it with other big data platforms (Section~\ref{section:implementation}). It supports several interactions for taking advantage of human perception and reasoning abilities in the visual analytics process (Section~\ref{section:interaction}).

\subsection{Data Clustering} \label{section:dataclustering}

We cluster the data points for each dimension (continuous variable) independently. For each dimension, there will be several clusters. One cluster represents that the data points in the cluster are close to each other in the dimension. These clustered points will be merged on the respective axis of a PCP.

We propose a one-dimensional clustering method especially for clustering the large-scale data in each dimension in a PCP, which is evolved from K-means clustering. K-means \cite{Wagstaf2001} automatically partition a data set into $k$ groups for a given data set $D=\left\lbrace  d_{1}, d_{2}, . . ., d_{n} \right\rbrace$ as follows:
\begin{enumerate}
	\item Select $k$ initial cluster centers, $C_{1}, C_{2}, . . ., C_{k}$.
	\item For each point $d_{i}$ in the data set $D$, assign it to the closest cluster $C_{j}$ by computing the least squared Euclidean distance.
	\item For each cluster $C_{i}$, update its center by averaging all of the points $d_{j}$ that have been assigned to it.
	\item Iterate between (2) and (3) until convergence.
	\item Return $k$ clusters, $\left\lbrace C_{1}, C_{2}, . . ., C_{k}\right\rbrace$. 
\end{enumerate}

The K-means algorithm converges when there is no further change in assignment of instances to clusters by using an iterative refinement technique. For one-dimensional data, K-means will generate several ordered clusters with different size and without overlap. Arthur and Vassilvitskii have proved that the worst-case running time of the method is exponential in the number of points \cite{arthur2006slow}. Therefore, it is hard to be applied in the visual analytics process directly for a large-scale data set.

To address this challenge, instead of selecting $k$ random initial cluster centers, we specifically set $k$ selected fixed centers. Then we modify K-means clustering with the following two considerations to eliminate the iterations in the algorithm:
\begin{enumerate}
	\item In a parallel coordinates plot, the data points in each axis are ordered and one point will be only grouped into one cluster.
	\item For a complex data set, to take advantage of human reasoning, perception, and cognition, users may prefer to specify the clusters based on their own knowledge than an automated algorithm.
\end{enumerate}

With the first consideration, for a specified cluster number $k$, the clusters in one axis are also ordered and there is no overlap between clusters, which is illustrated in Figure~\ref{fig:clustersinaxis}. In Figure~\ref{fig:clustersinaxis}, we use a center and a radius to define a cluster in one axis, where the gray rectangles represent clusters, the blue dots represent the centers of the clusters, and the green lines represent the radius of the clusters. With this definition, $k$ clusters in one axis  for a given data set $D$ are expressed as follows:
% \[ 
% \left\lbrace (C_{1},R_{1}), (C_{2},R_{3}), . . ., (C_{k},R_{k}) \mid C_{i}<C{i+1}, R_{i} \leq C_{i+1} - C_{i}, \sum_{i=1}^{k} R_{i} \leq %(d_{max}-d_{min})/2
%  \right\rbrace 
%\]
\[
\left\lbrace (C_{1},R_{1}), (C_{2},R_{3}), . . ., (C_{k},R_{k})\right\rbrace 
\]
which fulfills the following constrains:
\[
C_{i}<C_{i+1}, R_{i} \leq C_{i+1} - R_{i+1} - C_{i}, \sum_{i=1}^{k} R_{i} \leq (d_{max}-d_{min})/2
\]
where $C_{i}$ is the center of the $i$-th cluster, $R_{i}$ is the radius of the $i$-th cluster, $d_{max}$ is the maxima of the data set $D$, and $d_{min}$ is the minima of the data set $D$. 
  
In our method, to cluster the data in a given data set $D$ into $k$ groups, we first specifically select $k$ fixed centers which evenly divides the data set. Accordingly, for a given data set $D$, we can compute $k$ ordered clusters with the same radius without iterations through the following computation:
\[
C_{i}=d_{max}-R\times(1+2\times i), R = \frac{(d_{max}-d_{min})}{2 \times k}
\] 
This computation only relies on the maxima, minima of the data set and the number of the clusters. This will reduce much computation time that needed for other clustering method \cite{Palmas2014} used in edge-bundling PCPs.

Furthermore, for complex data sets, the clusters with the same size may be not enough for exploring the data and gaining insight into the data. Based on the second consideration, for taking advantage of human perception and reasoning abilities, our method allow users to specify the number of clusters, and the centers and the various radiuses of the clusters in one axis, as long as the the specified parameters fulfill the condition in the previously mentioned formula. This visual analytics process is demonstrated in Section~\ref{section:experiment}.

Categorical variables are not clustered using the above method. Instead, we treat each category as a cluster. Using this method, the time of computing arbitrary clusters for a large-scale data set could be ignored with the known maxima and minima. The efficient process of obtaining maxima and minima of a extreme large-scale data set is discussed in Section~\ref{section:implementation}. 


\begin{figure}[tb]
	\centering
	\includegraphics[width=.8\linewidth]{imgs/axis-cluster}
	\caption{\label{fig:clustersinaxis}
		\textit{Clusters in one (horizontal) axis of a PCP.}}
\end{figure} 

\subsection{Edge Merging} \label{section:edgemerging} 

In a classic PCP, the data points are drawn as polylines. Our method merges these polylines according to the clusters in each axis into one single line and renders the merged line as a cubic B\'ezier spline with a specific width. The width is determined by the density information of the merged line. The purpose of our edge-merging method is to provide a more informative visualization of the internal structure of the clusters and the data distribution between axes, and reduce rendering time in order to interactively and visually explore a large-scale data set. The idea of our edge-merging method combines edge bundling in PCP and confluent drawing which is illustrated in Section~\ref{section:related work}. We use B\'ezier splines because they are widely used in edge-bundling PCP to guarantee $C^{1}$ continuous, which are also easy to follow with the eyes. 

To formulate and discuss our edge-merging method, we first denote the clusters in one axis as: $C_{A}^{k}$, where $A$ refers to the name of the axis, $k$ represents that it is the $k$-th cluster in this axis. A B\'ezier spline that connects the centers of two clusters in two axes is denoted as: $B(C_{A}^{i}, C_{B}^{j})$. A pair of two clusters in two axes are denoted as: $P(C_{A}^{i}, C_{B}^{j})$. If the data points $a$ in axis $A$ and $b$ in axis $B$, and $a\in C_{A}^{i}$ and $b\in C_{B}^{j}$, we define it as data points belong to a pair of clusters, denoted as $(a,b) \in P(C_{A}^{i}, C_{B}^{j})$. The number of data points that belong to $P(C_{A}^{i}, C_{B}^{j})$ is denoted as: $N(C_{A}^{i}, C_{B}^{j})$. Then, we describe our edge-merging method by actually drawing an example PCP with two axes, two clusters, and several data points, as illustrated in Figure~\ref{fig:edgemerging}. Consider there are two neighboring axes A and B, and two clusters $C_{A}^{1}$ and $C_{B}^{1}$ in the two axes. With a classic PCP, data points that belong to the two clusters are drawn as polylines, as illustrated in Figure~\ref{fig:edgemergingC}. In Figure~\ref{fig:edgemergingO}, with our edge-merging method, all polylines belong to these two clusters are merged together as one single B\'ezier spline with a specific width, which starts from the center of cluster $C_{A}^{1}$ and ends at the center of cluster $C_{B}^{1}$ and denoted as $B(C_{A}^{1}, C_{B}^{1})$. 

\begin{figure}[tb]
	\centering
	\begin{subfigure}{0.6\linewidth}
		\centering
		\includegraphics[width=.6\linewidth]{imgs/edgemerging1}
		\caption{\label{fig:edgemergingC}
			\textit{Several polylines between two neighboring axes in a classic PCP.}} 
	\end{subfigure}
	%\par\bigskip
	%\hspace*{\fill} 
	\begin{subfigure}{0.6\linewidth}
		\centering
		\includegraphics[width=.6\linewidth]{imgs/edgemerging2}
		\caption{\label{fig:edgemergingO}
			\textit{Several polylines merged as one single B\'ezier spline.}}
	\end{subfigure}
	
	\caption{\label{fig:edgemerging}
		\textit{Edge merging between two axes A and B.}}
\end{figure} 

In our approach, there is a maximum of $k_{A}\times k_{B}$ merged lines between two neighboring axes, where $k_{A}$ and $k_{B}$ are the number of clusters in either axis. For each merged line, we also compute its density, which is used to specify its width, as follows:
\begin{enumerate}
	\item For each two neighboring axes $A$ and $B$, compute clusters in either axis: $C_{A}^{i}$ and $C_{B}^{j}$.
	\item For $C_{A}^{i}$ and $C_{B}^{j}$, compute all pairs of clusters between the two axes with data points: $P(C_{A}^{i}, C_{B}^{j})$.
	\item For two data points $a$ and $b$ in the two axes, if $(a,b) \in P(C_{A}^{i}, C_{B}^{j})$,  $N(C_{A}^{i}, C_{B}^{j})$ add one.
	\item Iterate the step (3) for all data points in the two axes.
	\item Compute the density of $B(C_{A}^{i}, C_{B}^{j})$ by: $\frac{N(C_{A}^{i}, C_{B}^{j})}{\sum_{i=1}^{i}\sum_{j=1}^{j}N(C_{A}^{i}, C_{B}^{j})}$
\end{enumerate}

As shown in Figure~\ref{fig:edgemerging}, $N(C_{A}^{1}, C_{B}^{1})$ is 5, and the density of $B(C_{A}^{1}, C_{B}^{1})$ is 1. In our edge-merging method, $B(C_{A}^{i}, C_{B}^{j})$ and $N(C_{A}^{i}, C_{B}^{j})$ are used for rendering the merged lines (see in Section~\ref{section:representation}).


\subsection{Representation} \label{section:representation}

In classic PCPs, drawing the polylines or curves for each data point has two main disadvantages for a large-scale data set:
\begin{itemize}
	\item  Visual clutter and overplotting which hampers the recognition of patterns and trends in the data.
	\item The rendering performance depends on the number of data points so that large-scale data sets cannot be explored interactively.
\end{itemize} 
These disadvantages are also true for an edge-bundling PCP since they still need to render each data point as a polyline or a curve. Furthermore, with edge bundling, the polylines or curves may be closer, which actually somehow increases the visual clutter and overplotting of the bundled lines or curves.

To address these challenges, we merge data points that belong to a pair of clusters in two axes as one single B\'ezier spline, which connects the centers of two clusters. Based on the clustering result, we render a merged B\'ezier spline between axes as illustrated in Figure~\ref{fig:edgemergingO}. We compute the density of a merged B\'ezier spline to determine its width as follows:
\[ 
W_{b} = D \times W_{max}
 \]
 where, $W_{b}$ is the width of the merged B\'ezier spline $B(C_{A}^{i}, C_{B}^{j})$, $D$ is the density of the merged B\'ezier spline, $W_{max}$ is the max line width in the whole visualization. For different data sets, $W_{max}$ is configurable. Figure~\ref{fig:densityRepresent} shows the comparison of a classic PCP with the PCP using our edge-merging layout and density based rendering methods. Since the total density of all merged lines between two axes is 1, in our edge-merging layout, the width of a merged line reflects the distribution of data points between the axes.
 
 \begin{figure}[tb]
 	
 	\centering
 	\begin{subfigure}{1\linewidth}
 		\centering
 		\includegraphics[width=1\linewidth]{imgs/car1}
 		\caption{\label{fig:densityRepresentC}
 			\textit{Classic parallel coordinate plot.}} 
 	\end{subfigure}
 	%	\hspace*{\fill} % separation between the subfigures
 	\par\bigskip
 	\begin{subfigure}{1\linewidth}
 		\centering
 		\includegraphics[width=1\linewidth]{imgs/car2}
 		\caption{\label{fig:densityRepresentO}
 			\textit{PCP using our edge-merging with density-based rendering.}}
 	\end{subfigure}
 	
 	\caption{\label{fig:densityRepresent}
 		\textit{Comparison of the classic PCP and the edge-merging PCP on a car data set.} }
 \end{figure} 

 It is easy to see that our edge-merging layout has a much smaller visual footprint than a classic PCP. With fewer B\'ezier splines, it not only reduces visual clutter and overplotting but also reduces the rendering time. More importantly, the rendering performance of our edge-merging layout is independent of the number of data points since we only render the merged B\'ezier spline, which is demonstrated in Section~\ref{section:experiment}. For two given axes, the maximum of merged lines between them only depends on the number of clusters in each axis. Compared with the number of data points in a large-scale data set, the number of merged lines between two axes with a give configuration of clustering is much smaller and constant. Therefore, our edge-merging layout is scalable for large-scale data sets.


\subsection{Implementation} \label{section:implementation}
We implement our edge-merging technique in a web-based visual analytics application with an intention to integrate it with other big data platforms. It is implemented in Java using spring MVC framework \cite{Ladd2006}, and JavaScript using Data-Driven Documents (D3) \cite{bostock2011d3}.  It supports the visual analytics process by providing several interactions including configuring the clustering and changing the order of axes, which are described in Section~\ref{section:interaction}. The visual analytics and knowledge generation process of the application is shown in Figure~\ref{fig:process}. 

\begin{figure}[tb]
	\centering
	\includegraphics[width=1\linewidth]{imgs/process}
	\caption{\label{fig:process}
		\textit{The visual analytics and knowledge generation process of the visual analytics application.}}
\end{figure} 

According to Figure~\ref{fig:process}, the web-based architecture of our application separates the rendering process and clustering process. The clustering process, which takes most of the computation time, is performed on the server side. It will reduce the transmission time of data in the network since the data are stored in a relational database or big data platforms in servers. The rendering process is performed in clients' browsers lightweight based on the clustering result. This separation allows users to interactively explore large-scale data with an edge-merging PCP in their browsers, because the clustering result, which contains few graphical elements, could be rendered in browsers in real time.

One additional advantage of our implementation is that it could take advantage of the state-of-the-art advances in data processing and management technologies on the server side. First, the computation is independent for each data item. Therefore, the process can be parallelized: the clustering can be run either on a GPU (which can handle more than 1000 items in parallel) or on a distributed platform such as Apache Hadoop. Second, the results of the clustering process are small in size. Therefore, extensive caching and precomputation can be used. When the user chooses a particular cluster configuration, the clustering must be done only once. Afterwards, the result of the clustering can be cached on the server in a relational database or memory. Next time when a visualization with the same cluster configuration is needed, it can be loaded from the cache immediately. In addition, the server can precompute likely configurations that the user will explore. In this way, the user would experience real-time interaction without any delays.

%In the application, data sets are stored in a relational database and different types of data could be processed automatically. In addition, large-scale data sets could be stored in big data platforms. According to Figure~\ref{fig:process}, the clustering process, which takes most of the computation time, is performed on the server side. For extreme large-scale data, it can be optimized in several ways. First, the computation is independent for each data item. Therefore, the process can be parallelized: the clustering can be run either on a GPU (which can handle more than 1000 items in parallel) or on a distributed platform such as Apache Hadoop. Second, the results of the clustering process are small in size. Therefore, extensive caching and precomputation can be used. When the user chooses a particular cluster configuration, the clustering must be done only once. Afterward, the result of the clustering can be cached on the server in a relational database or memory. Next time when a visualization with the same cluster configuration is needed, it can be loaded from the cache immediately. In addition, the server can precompute likely configurations that the user will explore. In this way, the user would experience real-time interaction without any delays.

%One additional advantage of our implementation is that the rendering process of the visualization is performed in browsers, which separate the 
 %the visualization contains few graphical elements. That makes the rendering process in the browser lightweight. Therefore, the chart can be made interactive. 
%For example, if the user chooses many clusters for some axes, the visualization can become cluttered. While this should rarely happen in practice, it is up to the user to choose the number of clusters. To help decrease the clutter in case of many clusters, the user could manually realign the curves between the axes. This would not be possible for a classic PCP. The number of lines in it would be so large, that an interactive version of a PCP with many data items would not be realistic in a web browser.

%Our visual analytics framework is a general web application, which is implemented in Java using spring MVC framework \cite{Ladd2006}, and JavaScript using Data-Driven Documents (D3) \cite{bostock2011d3}. It could be used to visually explore various high-dimensional data sets. It supports to render large-scale data sets in an edge-merging layout for PCP. The knowledge generation process of this visual analytics framework is shown in Figure~\ref{fig:process}. According to Figure~\ref{fig:process}, this framework integrates human perception ability and expertise through the interaction (described in Section~\ref{section:interaction}) to configure the clustering process and generating corresponding edge-merging PCP. Furthermore, for extreme large-scale data sets, the computation of clustering could also be performed in big data platforms to accelerate the clustering process. According to the clustering algorithm described in Section~\ref{section:cluster}, the clustering process could be easily transferred to several SQL statements, including selecting the maxima and minima values, counting the numbers of each cluster (grouping statement in where clause). The clustering result could be sent to the server through web services.


\subsection{User Interactions} \label{section:interaction}

Our application allows users to interactively explore the visualization space through a control panel that is shown in Figure~\ref{fig:controlPanel}. The application provides the following interactions:
\begin{description}
	\item [(a)] Users will select one data set from a list of data sets in the system. These data sets can be stored in a relational database, such as MySQL, or a big data platform, such as Apache Hadoop.
	\item [(b)] For each axis, users will specify and save the clustering configuration. Users will first select one axis from a list of all dimensions. Then input the number of clusters $n$, and the center and the radius of each cluster in order by the format: $C_{1},R_{1};C_{2},R_{2};...;C_{n},R_{n}$, where $C$ is the center of the cluster and $R$ is the radius of the cluster. Finally, users will save the configuration.
	\item[(c)] Users will input the names of dimensions (axes) by the format: $name_{1},name_{2},...,name_{n}$, and save the configuration. The application only visualizes the data for the input dimensions. The data for each dimension will be visualized in order of the input names. Therefore, the input information is used for adding and deleting axes and changing the order of axes.
	%Users will input the names of axes by the format: $name_{1},name_{2},...,name_{n}$, and save the configuration. Users can choose which axes will be visualized since the application only visualizes the data with the input names. Furthermore, the axes will be visualized in order of the input names. Therefore, the input information is also used for changing the order of the axes.
	\item[(d)] System will update the visualization according to the users' interactions and the saved configurations.
\end{description}

\begin{figure}[tb]
	\centering
	\includegraphics[width=0.8\linewidth]{imgs/control_panel_areas}
	\caption{\label{fig:controlPanel}
		\textit{The control panel of the visual analytics application. (a) Data sets selection. (b) Clustering configuration. (c) Coordinates configuration. (d) Visualization update.}}
\end{figure} 


\section{Experimental Results} \label{section:experiment}
In this section, we demonstrate the effectiveness of our edge-merging PCP technique through experiments on several data sets.

First, we examined the effectiveness of our edge-merging PCP on a wholesale customer data set from the UCI Machine Learning Repository. The data set refers to customers of a wholesale distributor, which includes the annual spending in monetary units (m.u.) on 6 product categories \cite{Baudry2015}. In Figure~\ref{fig:wholesale}, 3 selected variables of the data set are visualized. Figure~\ref{fig:wholesale2} is the clustering and edge-merging result over the classic PCP shown in Figure~\ref{fig:wholesale1} of the data set. In Figure~\ref{fig:wholesale1}, due to the visual clutter and the overlap of data items, it hides the patterns in the data set and reveals some incorrect results. For example, it shows that the numbers of customers for delicatessen products are almost the same from the Horeca and the Retail channel. The distribution of delicatessen products into geographical regions (Lisbon, Oporto and Other) is not clear from the plot. In contrast, our edge-merging PCP shown in Figure~\ref{fig:wholesale2} successfully reveals the hidden patterns in the data set and shows the trends and the data distribution between axes.
% , which are hard to be revealed through other existing edge-bundling methods.
It reduces visual clutter and the overlap of data items by rendering the width of the merged curves according to their densities. 
% According to Figure~\ref{fig:wholesale2}, 
For example, the number of customers for delicatessen products from the Horeca channel is about twice that from the Retail channel (while it seemed to be similar in Figure~\ref{fig:wholesale1}). It also shows data distribution between the different regions in detail. In addition, our result also successfully shows the major clusters and outliers (rare items or observations which raise suspicions by differing significantly from the majority of the data \cite{Zimek2017}) even without the assistance of the color and opacity channels. In our result, the data items with extreme small proportions are visualized as dashed lines. For example, 
% in Figure~\ref{fig:wholesale2}, 
the red dashed lines show that very few costumers spend more than 17980.5 m.u. on delicatessen products annually.

\begin{figure}[tb]
	
	\centering
	\begin{subfigure}{1\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{imgs/wholesale}
		\caption{\label{fig:wholesale1}
			\textit{Classic parallel coordinate plot.}} 
	\end{subfigure}
	\par\bigskip
	\begin{subfigure}{1\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{imgs/wholesale2}
		\caption{\label{fig:wholesale2}
			\textit{With the data clustering and the edge-merging layout.}}
	\end{subfigure}
	
	\caption{\label{fig:wholesale}
		\textit{Experiments on a wholesale customers data set with 3 dimensions and 440 data items.}}
\end{figure}

Next, we tested our proposed methods on a more sophisticated multi-dimensional data set within the visual analytics process. A widely used car information data set with seven variables is visualized in Figure~\ref{fig:experiment}.
%, which is widely used in many previous publications \cite{peng2004clutter}, is visualized. 
Original plot, based on a classic PCP, is shown in Figure~\ref{fig:experiment1}. Figure~\ref{fig:experiment2} shows PCP with edge-merging and automatic clustering, based on the same data set. The clusters in each dimension have the same size, which is computed without human judgment according to the default number of clusters for each dimension. Comparing Figure~\ref{fig:experiment1} and Figure~\ref{fig:experiment2}, our edge-merging layout for PCP successfully shows the major clusters, outliers, and the data distribution between axes even without the assistance of the color and opacity channels. For example, in Figure~\ref{fig:experiment2}, the red dashed lines could be seen as outliers because their proportions are too small compared with others. The well-organized B\'ezier splines and clear distribution between the axes of mpg, cylinders, and displacement reveal the following patterns and trends about the data set:
\begin{enumerate}
    \item Most cars' mpg attributes are equally distributed around 27.79 and 15.25, only a relatively small proportion of this attribute values lie around 40.33.
    \item Cylinders attributes are near equally distributed around  6.75 and 4.25.
    \item Most cars with mpg around 27.79 have cylinders around 4.25 and most cars with mpg around 15.25 have cylinders around 6.75.
    \item All cars with cylinders around 4.25 have displacement around 132.5.
    \item Cars with cylinders around 6.75 have displacement mainly around 261.5 and 390.5.
\end{enumerate}
    

In Figure~\ref{fig:experiment2}, the trends and data distributions between the axes of horsepower, weight, and acceleration are still not clear enough. In the visual analytics process, this could be improved by taking advantage of human perception and reasoning abilities. After obtaining a perception of data trends and the distributions between axes of horsepower, weight, and acceleration based on Figure~\ref{fig:experiment2}, we configure the new clustering of these axes, which is shown in Figure~\ref{fig:experiment3}. Comparing Figure~\ref{fig:experiment3} and Figure~\ref{fig:experiment2}, the pattern and data distribution in Figure~\ref{fig:experiment3} made with human judgment are better revealed compared to Figure~\ref{fig:experiment2}. It shows that a big proportion of cars have horsepower around 73 and a relatively small proportion of cars have horsepower around 150. Most cars weigh between 2000 and 4000, and have acceleration attributes around 15.

%As illustrated, the edge-merging layout can enhance the patterns with the data and reveal the trends and data distribution between axes. It reduces much visual clutters and overplotting for large-scale data sets. Accordingly, the color and opacity channels can be spared for representing other information. More importantly, our visual analytics framework can integrate human perception and reasoning abilities into the data analysis process to continuously improve the visualization results.

\begin{figure}[tb]
	\centering
	\begin{subfigure}{1\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{imgs/ex}
		\caption{\label{fig:experiment1}
			\textit{Classic parallel coordinate plot.}} 
	\end{subfigure}
	\par\bigskip
	\begin{subfigure}{1\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{imgs/e1}
		\caption{\label{fig:experiment2}
			\textit{With edge-merging layout and automatic data clustering.}}
	\end{subfigure}
\par\bigskip
\begin{subfigure}{1\linewidth}
	\centering
	\includegraphics[width=1\linewidth]{imgs/e2}
	\caption{\label{fig:experiment3}
		\textit{With edge-merging layout and manually clustering.}}
\end{subfigure}
	
	\caption{\label{fig:experiment}
		\textit{Experiments on a car data set with seven dimensions and 392 data items.}}
\end{figure} 

Our technique is scalable for large-scale data. Figure~\ref{fig:carm} shows a synthesized data set based on the car data set, which has seven dimensions and $10^{5}$ data items. In Figure~\ref{fig:carm1}, the data set is visualized in a classic PCP. In Figure~\ref{fig:carm2}, the data set is visualized in a PCP with edge-merging layout and three clusters in each dimension. The comparison between Figure~\ref{fig:carm1} and~\ref{fig:carm2} clearly shows that our technique reveals the data trends, patterns and distributions between clusters, and greatly reduces visual clutter. 

To further illustrate the effectiveness of our edge-merging technique, we analyze its running time of its clustering and rendering process with several synthesized five-dimensional data sets. The synthesized data sets were randomly generated based on the wholesale customers data set and the car data set. The application was implemented on a MacBook Pro desktop with 3.1 GHz Intel Core i5 CPU, 8GB Memory and Intel Iris Plus 650 Graphics Processing Unit (GPU). 
\begin{figure}[tb]
	\centering
	\begin{subfigure}{1\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{imgs/carm}
		\caption{\label{fig:carm1}
			\textit{Classic parallel coordinate plot.}} 
	\end{subfigure}
	\par\bigskip
	\begin{subfigure}{1\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{imgs/carm2}
		\caption{\label{fig:carm2}
			\textit{With edge-merging layout and three clusters in each dimension.}}
	\end{subfigure}
	
	\caption{\label{fig:carm}
		\textit{Experiments on a synthesized car data set with seven dimensions and $10^{5}$ data items.}}
\end{figure} 

First, a run-time analysis of the clustering algorithm with the synthesized data sets was performed. The clustering algorithm includes the process of computing the clusters and the densities (described in Section~\ref{section:dataclustering} and~\ref{section:edgemerging}). In the test, the default number of clusters was set to five. For each data set with different data items, the clustering algorithm was executed ten times and the average running time was calculated. According to the result shown in Table~\ref{tab:run-time}, the proposed clustering algorithm is scalable for large-scale data. Its running time increases linearly with the number of data items. Furthermore, the running time of the proposed clustering algorithm is much shorter compared with other clustering algorithms used in PCP. For example, Palmas et al. \cite{Palmas2014} present a density-based clustering for each dimension independently in edge-bundling PCP, which takes about one minute for clustering a one-dimensional data set with $10^{5}$ data items. In contrast, our algorithm takes 1.20980 seconds for clustering a five-dimensional data set with $10^{5}$ data items, which allows the interactive use of it in the visual analytics process.
%By reducing much computing time for clustering data, our clustering method could be interactively used in the visual analytics process.

\begin{table}[tb]
	\caption{\textit{Run-time analysis of the clustering algorithm.}}
	\label{tab:run-time}
	%\scriptsize%
	\centering%
	\begin{tabu}{%
			c c
		}
		\toprule
		Number of data items & Run-time (s) \\
		\midrule
		$10^{3}$ & 0.06820 \\
		$10^{4}$ & 0.14610 \\
		$5\times10^{4}$ & 0.63520 \\
		$10^{5}$ & 1.20980 \\
		$5\times10^{5}$ & 6.08090 \\
		$10^{6}$ & 15.01720 \\
		\bottomrule
	\end{tabu}%
\end{table}

Next, we analyze the rendering time of our edge-merging PCP based on the synthesized data sets. The clustering time described above depends on the performance of the server where data processing is running. In contrast, rendering time needed to draw the chart in the web browser depends on the computing power of the user's computer. As described earlier, the proposed solution is scalable - the clustering and rendering processes can be distributed on different computers. To make the comparison of rendering time in our edge-merging PCP and a classic PCP fair, only time for rendering the data items is included. The time for rendering the axes, labels, and stickers are not included - this part is static and requires a constant rendering time regardless of the number of data items. The result is shown in Table~\ref{tab:render-time}. According to Table~\ref{tab:render-time}, the rendering time of our edge-merging PCP is much shorter compared to that of classic PCP. It allows our edge-merging PCP to be interactively used in the visual analytics process. More importantly, the rendering performance of our edge-merging PCP remains nearly constant when the number of data items increases. In fact, its rendering depends only on the cluster configuration, not the number of data items. It makes our edge-merging technique scalable for large-scale data sets. For data sets with more than $10^{5}$ items, the classic PCP takes more than one minute and often causes a crash in browsers. In contrast, our edge-merging PCP still takes less than 0.001 seconds for rendering these data sets.


\begin{table}[tb]
	\caption{\textit{Rendering time analysis of the edge-merging layout.}}
	\label{tab:render-time}
	%\scriptsize%
	\centering%
	\begin{tabu}{%
			M{2cm} M{2.5cm} M{2.5cm}
		}
		\toprule
		Number of data items & Rendering time (s) of the classic PCP & Rendering time (s) of the edge-merging PCP \\
		\midrule
		$10^{3}$ & 0.03279 & 0.00097 \\
		$10^{4}$ & 0.28104 &  0.00088 \\
		$5\times10^{4}$ & 1.50314 &  0.00092 \\
		$10^{5}$ & 3.00769 &  0.00094 \\
		\bottomrule
	\end{tabu}%
\end{table}

\section{Discussions} \label{section:discussion}

From the experiments, we can see that our edge-merging PCP has clear advantages for the visual analytics process, especially when the size of data is scaled up. Firstly, it greatly reduces visual clutter. It helps to reveal the trends, hidden patterns and data distributions between axes. Furthermore, compared with other edge-bundling PCP, it supports the interactive use in the visual analytics process for large-scale data. The performance is acceptable for near-real-time interaction. Its computing time of the clustering process is linearly increased with the number of data items, which is much shorter than other edge-bundling PCP optimizations. Its rendering performance is independent of the number of data items. Therefore, our edge-merging PCP is scalable for large-scale data. Finally, it allows users to integrate their perception and reasoning abilities into the data analysis process by supporting the configurable clustering.
%Finally, the web-based architecture of the application could be extended with other big data platforms. 

Although our application supports the interactions of changing the order of axes, adding and deleting axes, and configuring the number and size of clusters, one limitation of the current version is that all interactions are performed through a control panel, which is not intuitive for users.

\section{Conclusion and Future Work}\label{section:future}
In this paper, we present a novel edge-merging PCP for visual exploration of large-scale multi-dimensional data sets. Based on the edge-merging PCP, we implement a web-based visual analytics application, which could be extended with other big data platforms to supports extreme large-scale data sets. In the edge-merging technique, we propose a one-dimensional clustering method which is evolved from K-means. The edge-merging PCP merges data points based on the clustering to reduce visual clutter caused by overplotting. It uses density information to render the merged B\'ezier splines to reveal the trends and data distributions between axes, which leaves the color and opacity perceptual channels free for visualizing other information. Furthermore, its clustering algorithm has linear complexity and the rendering performance of its edge-merging layout is independent of the number of data points, which makes it available for the interactive usage in the visual analytics process. More importantly, this visual analytics application integrates human perception and reasoning abilities into the data analysis process by supporting the configuration of the clustering in each axis to continuously improve the visualization results. 
%This framework could integrate with other big data platforms through web services to support extreme large-scale data sets. 
 
The work in this paper can be further improved in several ways. In the current implementation, the interactions are performed through a control panel. We plan to develop more intuitive interactions for this framework. In addition, a controlled user study could be done in the future to evaluate the usability of the framework. To improve the visualization, the color and opacity perceptual channels could be investigated for display of additional information. 

%-------------------------------------------------------------------------

==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

